Sequence-based Machine Learning Models in Jet Physics

Sequence-based modeling broadly refers to algorithms that act on data that is represented as an ordered set of input elements. In particular, Machine Learning algorithms with sequences as inputs have seen successfull applications to important problems, such as Natural Language Processing (NLP) and speech signal modeling. The usage this class of models in collider physics leverages their ability to act on data with variable sequence lengths, such as constituents inside a jet. In this document, we explore the application of Recurrent Neural Networks (RNNs) and other sequence-based neural network architectures to classify jets, regress jet-related quantities and to build a physics-inspired jet representation, in connection to jet clustering algorithms. In addition, alternatives to sequential data representations are briefly discussed.

==> text/diag_lstm.tex <==
\begin{figure}
\begin{center}
\begin{tikzpicture}

\draw [rounded corners] (-3.5,0) rectangle (-0.5,2);

\draw [rounded corners] (0,0) rectangle (3,2);

\draw [rounded corners] (3.5,0) rectangle (6.5,2);


% \draw[black,thick] (-2,0) circle[radius=0.5] ;
% \draw[black,thick] (0,0) circle[radius=0.5] ;
% \draw[black,thick] (2,0) circle[radius=0.5] ;
% \draw[->, thick] (-3.5,0) -- (-2.5,0);
% \draw[->, thick] (-1.5,0) -- (-0.5,0);
% \draw[->, thick] (0.5,0) -- (1.5,0);
% \draw[->, thick] (2.5,0) -- (3.5,0);
% \draw (-2,0) node {$\mathbf{x}^{t-1}$};
% \draw (0,0) node {$\mathbf{x}^{t}$};
% \draw (2,0) node {$\mathbf{x}^{t+1}$};
% \draw (-3,0.25) node {$f$};
% \draw (-1,0.25) node {$f$};
% \draw (1,0.25) node {$f$};
% \draw (3,0.25) node {$f$};
\end{tikzpicture}
\caption{Scheme of a sequence-based algorithm acting on a sequence of inputs $\mathbf{x}^{t}$.}
\label{fig:lstm_arch}
\end{center}
\end{figure}
